LLM as a System Service on Mobile Devices

Being more powerful and intrusive into user-device interactions, LLMs are eager for on-device execution to better preserve user privacy. In this work, we propose a new paradigm of mobile AI: LLM as a system service on mobile devices (LLMaaS). Unlike traditional DNNs that execute in a stateless manner, such a system service is stateful: LLMs execution often needs to maintain persistent states (mainly KV cache) across multiple invocations. To minimize the LLM context switching overhead under tight device memory budget, this work presents LLMS, which decouples the memory management of app and LLM contexts with a key idea of fine-grained, chunk-wise, globally-optimized KV cache compression and swapping. By fully leveraging KV cache's unique characteristics, it proposes three novel techniques: (1) Tolerance-Aware Compression: it compresses chunks based on their measured accuracy tolerance to compression. (2) IO-Recompute Pipelined Loading: it introduces recompute to swapping-in for acceleration. (3) Chunk Lifecycle Management: it optimizes the memory activities of chunks with an ahead-of-time swapping-out and an LCTRU (Least Compression-Tolerable and Recently-Used) queue based eviction. In evaluations conducted on well-established traces and various edge devices, \sys reduces context switching latency by up to 2 orders of magnitude when compared to competitive baseline solutions.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> fig-LLMaaS.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.47\textwidth]{figs/LLMaaS.pdf}
    \caption{On-device LLM as a Mobile OS Service.}
    \label{fig:LLMaaS}
\end{figure}

==> fig-LLMaaS_moti.tex <==
\begin{figure}[t]
  % \centering
  % \begin{minipage}[b]{0.20\textwidth}
  %   \includegraphics[width=\textwidth]{figs/mem_LLMaaS.pdf}
  %   \vspace{-17pt}
  %   \subcaption{LLMaaS is mem.-effi.}
  %   \label{fig:mem-effi}
  % \end{minipage}
  % \hfill
  \begin{minipage}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/latency_energy_NPU.pdf}
    \vspace{-17pt}
    \subcaption{ASICs empower mobile AI.}
    \label{fig:ASIC_latency}
  \end{minipage}
  \begin{minipage}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{figs/op_LLMaaS.pdf}
    \vspace{-20pt}
    \subcaption{LLMaaS is friendly to mobile AI ASICs.}
    \label{fig:ASIC_op}
  \end{minipage}
  \vspace{-20pt}
  % \hfill
  \caption{Measurement results of hardware accelerator on mobile SoCs.
  Performed on MI14 with snapdragon 8Gen3 NPU and a state-of-the-art edge intelligence benchmark eAIBench~\cite{eAIBench}. 
  eAIBench has a vast coverage of mobile AI tasks and specific solution models.}
  \label{fig:measurement}
\end{figure}

==> fig-critical_path.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.47\textwidth]{figs/crop_critical_path.pdf}
    \caption{Execution paths of a context's memory managing activities.
    % (a) is a vanilla swapping method that permits swapping and allocation during LLM inference.
    % (b) is \sys's path-optimized method.
    % It forbids swapping 
    The green path is an overhead-optimal execution path; the red is overhead-worst. \mwx{this figure could be removed if out of space}}
    \label{fig:critical_path}
\end{figure}

==> fig-sys_model.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/sys_model.pdf}
    \caption{How \sys works.}
    \label{fig:sys_model}
\end{figure*}

==> sec-discussion.tex <==
\section{discussion}

batching/multi call

failure/interruption

one App multiple context

App activation overhead (once)

==> sec-trace.tex <==
\section{Context Switching Trace}
\label{sec: trace}

\input{tab-datasets}

% \mwx{Merge to implementation or experiment settings.}

To the best of our knowledge, there is no publicly available trace of LLMaaS context switching on devices.
In order to comprehensively and accurately evaluate \sys, we synthesized a trace that formulated by
\begin{equation}
    Trace = \{(Time_{i}, CtxtID_{i}, Prompt_{i}, groundTruth_{i})\},
\end{equation}
Where $Time_{i}$ is the $i_{th}$ calling time of \texttt{callLLM()} with $CtxtID_{i}$, and $Prompt_{i}$ and $groundTruth_{i}$ are the input and ideal output text.
Since the LLM we select for \service (7B-size) has enough zero-shot ability, we do not consider context-specific adapters here.
The prompts and groundTruths for a context are derived from a dataset in Table~\ref{tab:datasets}, while a dataset can derive multiple contexts.
We generate calling time $Time_{i}$ using Poisson distribution with different calling rates.
We consider three patterns of context switching:

\noindent $\bullet$~\texttt{Random}.
Contexts are switched with the same probability.

\noindent $\bullet$~\texttt{Markov}.
Context switching is determined by a first-order Markov process, which assigns higher priority to recently used contexts.

\noindent $\bullet$~\texttt{Gaussian}.
Context switching follows a Gaussian distribution w.r.t delta length. 
A context with moderate workload is more likely to be requested by the apps.

We synthesize 72-hours-long traces with different settings to evaluate \sys.
We will make the traces used in our experiments publicly available for reproducibility and further research on on-device LLMaaS.

